Graph Neural Network Bandits

We consider the bandit optimization problem with the reward function defined over graph-structured data. This problem has important applications in molecule design and drug discovery, where the reward is naturally invariant to graph permutations. The key challenges in this setting are scaling to large domains, and to graphs with many nodes. We resolve these challenges by embedding the permutation invariance into our model. In particular, we show that graph neural networks (GNNs) can be used to estimate the reward function, assuming it resides in the Reproducing Kernel Hilbert Space of a permutation-invariant additive kernel. By establishing a novel connection between such kernels and the graph neural tangent kernel (GNTK), we introduce the first GNN confidence bound and use it to design a phased-elimination algorithm with sublinear regret. Our regret bound depends on the GNTK's maximum information gain, which we also provide a bound for. While the reward function depends on all $N$ node features, our guarantees are independent of the number of graph nodes $N$. Empirically, our approach exhibits competitive performance and scales well on graph-structured domains.

==> older drafts/App0_details.tex <==
\section{Details of the Main Text}
\subsection{NN Definition and Relation to GNN}\label{app:nn_defs}
Let $f(\vx; \vtheta): \mathbb{R}^d \rightarrow \mathbb{R}$ be a fully-connected network, with $L$ hidden layers of equal width $m$, and ReLU activations, recursively defined as follows:
\begin{equation}
    \label{eq:def_nn}
    \begin{split}
        f^{(1)}(\vx) &= \mW^{(1)}\vx,\\
     f^{(l)}(\vx) &= \sqrt{\frac{2}{m}} \mW^{(l)} \sigma_{\text{relu}}\big(f^{(l-1)}(\vx)\big) \in \mathbb{R}^m, \,\, 1<l\leq L\\
    \nn(\vx; \vtheta) &= \sqrt{2} \mW^{(L+1)} \sigma_{\text{relu}}\big(f^{(L)}(\vx)\big)\in \sR.  
    \end{split}
\end{equation}
The weights $\mW^{(i)}$ are initialized to random matrices with standard normal i.i.d.~entries, and $\vtheta = (\mW^{(i)})_{i\leq L+1}$.% Let $\vg(\vx; \vtheta)=\nabla_\vtheta f(\vx; \vtheta)$ be the gradient of $f$.

According to the previous definition, the two layer NN with width $m$ is given as: 
\begin{equation} \label{eq:two_layer_nn}
    \nn(\vx; \vtheta) = \sqrt{2} \sum_{j=1}^m w_j^{(2)} \sigma_{\text{relu}}\big(
    \langle \vw_j^{(1)}, \vx \rangle \big),
\end{equation}
where $\vw_j^{(1)} \in \mathbb{R^d}$ are weights in the first layer and $w_j^{(2)} \in \mathbb{R}$ are weights in the second layer. Similarly, the two layer GNN (see \cref{eq:def_gnn}) is given by:
\begin{align}
    \gnn(G; \vtheta) &= \frac{1}{N} \sum_{u \in V(G)} \sqrt{\frac{2}{m}} \sum_{j=1}^m w_j^{(2)} \sigma_{\text{relu}}\big(
    \langle \vw_j^{(1)}, \bar{\vh}_u \rangle \big) \\
    &= \frac{1}{N} \sum_{u \in V(G)} \nn(\bar{\vh}_u; \vtheta), \label{eq:via_nn_def}
\end{align}
where \cref{eq:via_nn_def} follows from \cref{eq:two_layer_nn}. We note that the relation in \cref{eq:two_layer_nn} holds for arbitrary $L$.  

\subsection{Recursive expression for the NTK} \label{app:ntk_formula}
For the sake of completeness, we provide a closed-form expression for the NTK function used in \cref{eq:gntk_vs_ntk} (for more details, see Section 2.1 in \cite{bietti2020deep}). We limit the input space to $\mathbb{S}^{d-1}$ since, by the definition, our feature vectors are always normalized, i.e., $\|\bar{\vh}_u\|_2=1$ for every $u \in V(G)$. For a ReLU network with $L$ layers considered in \cref{eq:def_nn} with inputs on the sphere (by taking appropriate limits on the widths), the corresponding $\ntk(\vx, \vx')$ (\cite{jacot2018neural}) depends on $\angle (\vx,\vx')$ and is given by $\ntk(\vx, \vx') = \kappa^{(L)}_{\text{NN}}(\vx^T \vx')$ where
$\kappa^{(L)}_{\text{NN}}(\cdot)$ is defined recursively as follows:\looseness=-1

%, and $\ntk(x, x) = 1$.  Following \citet{bietti2020deep}'s notation, we define $\ntk(x, x') := k^{(L)}(x^Tx')$,
\begin{equation}
    \label{eq:ntk_formula}
\begin{split}
        \kappa_{\text{NN}}^{(1)}(u)&= \kappa^{(1)}(u) = u,  \\
        \kappa^{(l)}(u) & =  \kappa_1\big(\kappa^{(l-1)}(u)\big), \\
        \kappa_{\text{NN}}^{(l)}(u) & = \kappa_{\text{NN}}^{(l-1)}(u)\cdot \kappa_0\big(\kappa^{(l-1)}(u)\big) + \kappa^{(l)}(u) \quad \text{for } 2 \leq l \leq L,
        \end{split}
\end{equation}
where
\begin{align*}
\kappa_0(u) & = \frac{1}{\pi}\big(\pi-\arccos (u)\big),\\
\kappa_1(u) & = \frac{1}{\pi}\Big( u(\pi - \arccos(u)) + \sqrt{1-u^2} \Big).
\end{align*}
Finally, we note that $\kappa^{(L)}_{\text{NN}}(1) = 1$ (\citet{bietti2020deep}), and hence $\ntk(\vx, \vx') \leq 1$ for all $\vx,\vx' \in \mathbb{S}^{d-1}$.

% \subsection{Additive Structure of the GNTK}
% \label{sec:kernel_additive_structure}
% Define $\vx_G \in \sS^{Nd-1}$ as the stacked vector of all aggregated node features,
% \[
%     \vx_G = \Big(\bar\vh_{u}\Big)_{u \in V(G)}.
% \]

% Using this notation, we can re-write the definition of $\gntk$ as
% \begin{align}
%     \label{eq:additive_structure}
%     \gntk(G, G') & =
%     \underbrace{
%     \frac{1}{N^2} \sum_{i=1}^N  \ntk\big(\vx_{G, i:d(i+1)}, \vx_{G',i:d(i+1)}\big)}_{k_1(\vx_{G}, \vx_{G'})} \nonumber \\
%     &  + \underbrace{\frac{2}{N^2} \sum_{i=1}^N \sum_{{j=i+1}}^N \ntk\big(\vx_{G,i:d(i+1)}, \vx_{G',j:d(j+1)}\big)}_{k_2(\vx_{G}, \vx_{G'})}.
% \end{align}
% We note that $\gntk(G, G')$ can be written as the sum of the additive kernel $k_1(\vx_{G}, \vx_{G'})$ and additive kernel with overlapping groups $k_2(\vx_{G}, \vx_{G'})$. Maximum information gain bounds for these types of kernels are studied in \cite{kandasamy2015high} and \cite{rolland2018high}, respectively. The provided bounds hold when each member kernel (in the sum) is a stationary GP kernel (e.g., the squared-exponential kernel). Moreover, they do not consider the additional structure present in every lower dimensional group $\vx_{G,i:d(i+1)}$ in \Cref{eq:additive_structure}, i.e., $\vx_{G,i:d(i+1)} = \bar \vh_i = c_i\sum_{j \in \cN_G(i)} \vh_j$.

{\color{comment}\subsection{GNTK as direct sum of NTKs} \label{app:gnntrick}
In this section (and this section only) I'm using the additive model.
Before we dissect the connection between NTK and GNTK, we give a brief introduction into a network and its tangent kernel.

Set $\vtheta^0$ and consider the first order approximation of $\nn(\vx, \vtheta)$  and $\gnn(G, \vtheta)$ around the initial parameters $\vtheta^0$ 
\begin{align*}
    \tilde f_{\mathrm{NN}}(\vx, \vtheta) &= \gradnn^T(\vx, \vtheta^0)(\vtheta - \vtheta^0)^T,\\
    \tilde f_{\mathrm{GNN}}(G, \vtheta) &= \ggnn^T(G, \vtheta^0)(\vtheta - \vtheta^0)^T
\end{align*}
since the networks are defined to be zero at initialization. Consider any fixed dataset. Using a square loss, training with the linear model $\tilde f_{\mathrm{NN}}(\vx, \vtheta)$ (or $\tilde f_{\mathrm{GNN}}(G, \vtheta)$ resp.), is equivalent to regression with the {\em tangent kernel} \citep{jacot2018neural}, defined as 
\begin{align}
   \tilde k_{\mathrm{NN}} (\vx, \vx') & = \gradnn^T(\vx; \vtheta^0)\gradnn(\vx'; \vtheta^0),  \label{eq:finite_ntk} \\
   \tilde k_{\mathrm{GNN}} (G, G') & = \ggnn^T(G; \vtheta^0)\ggnn(G'; \vtheta^0)\label{eq:finite_gntk}
\end{align}
The tangent kernels are random, and depend on the network parameters. 
\citet{jacot2018neural} show that in the infinite width limit, $\tilde k_{\mathrm{NN}} (G, G')$ converges to a deterministic kernel, which they call the NTK,
\[
\lim_{m \rightarrow \infty} \tilde k_{\mathrm{NN}} (\vx, \vx')/m = \ntk(\vx, \vx').
\]
Similarly, we define the Graph Neural tangent kernel as 
\[
\gntk(G, G') := \lim_{m \rightarrow \infty} \tilde k_{\mathrm{GNN}} (G, G')/m.
\]
Next lemma proves that $\gntk$ is also deterministic and can be written as direct sums of $\ntk$ evaluated on aggregated features of different nodes of the graph.

\begin{lemma}\label{lem:main_gntk_ntk} Consider graphs $G$ and $G'$ with $N$ nodes. We use $\bar \vh_{G,j}$ to refer to the normalized aggregated feature of node $j$ in graph $G$.
\[
\gntk(G,G') = \frac{1}{N^2}\sum_{j,j' = 1}^N \ntk(\bar\vh_{G,j}, \bar \vh_{G',j'}) 
\]
\end{lemma}

% Let $P_N$ denote the set of permutations over an $N$-dimensional sequence, then $\vert P_N\vert = N!$.
% While members of $\Hgntk$ are invariance to neighborhood permutations on the input graph, they may not be invariant to permutations on the entire graph.
% To model a reward function that is invariant to permutation, we then work with the smoothed GNTK,
% \begin{equation}
%     \gntkbar(G, G') = \frac{1}{N!} \sum_{c \in P_N} \gntk(c \cdot G, G')
% \end{equation}
% Let $\Hgntkbar$ denote the RKHS corresponding to $\gntkbar$. We now show that $f \in \Hgntkbar$ are invariant to node permutations.

\begin{proof}[\textbf{Proof of \cref{lem:main_gntk_ntk}}]
For any $\vtheta^0$ we first show that,
\begin{equation}\label{eq:finit_gntk_ntk}
\tilde k_{\mathrm{GNN}} (G, G') = \frac{1}{N^2} \sum_{j=1}^N \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j'}).
\end{equation}
Then we take the $m \rightarrow \infty$ limit.
%We consider functions $f: \cG \rightarrow \sR$ that are invariant to how the graph nodes are indexed, i.e. invariant to permutations on the graph. In this setting, the ordering of nodes in a neighbour does not change the effect of that neighborhood on the function value either. 

% ==================================================
% ==================================================
% Additive model proof
%===================================================
% ==================================================
The function $\gnn$ only operates on $G$ through its aggregated note features.
This motivates us to work with $\cX$ as the input domain where
\[
\cX = \left\{ \left(\bar\vh_{G,1}, \cdots,\bar\vh_{G,j}, \cdots, \bar\vh_{G,N} \right)\, \Big \vert \, \forall\, G \in \cG\right\} \subset \sR^{Nd}.
\]
Then $\cX = \bigcup_{j=1}^N \cX_j$, where $\cX_j = \{\bar \vh_{G, j} \vert \forall G \in \cG\} \subset \sR^{d, (j)}$ are $d$-dimensional subsets of $\sR^{Nd}$ and $\cX_j \cap \cX_i = \emptyset$ for all $i \neq j$.
By definition, we may write
\begin{equation}\label{eq:basic_def_gnn}
 \gnn(G; \vtheta^0) = \sum_{j=1}^N \frac{1}{N}\nn^{(j)}(\bar\vh_{G,j}; \vtheta^0)
\end{equation}
where the $(j)$ superscript is added to emphasize on the following: While the elements of $\vtheta^0$ are shared across the feed-forward networks, each $\nn^{(j)}: \cX_j \rightarrow \sR$ is zero outside $\cX_j$, if we extend its domain to $\cX$, i.e., for any $i \neq j$, 
\[
\nn^{(j)}(\bar \vh_{G, i}; \vtheta^0) = 0.
\]
Further, for any $G$, the gradient vectors $\gradnn^{(j)}(G; \vtheta^0) \in \sR^{d, (j)}$ reside in orthogonal subsets of $\sR^{Nd}$ and therefore for any $i\neq j$ and graphs $G, G' \in \cG$,
\begin{equation} \label{eq:grad_innerprod_zero}
\langle  \gradnn^{(i)}(\bar \vh_{G,i}), \gradnn^{(j)}(\bar \vh_{G',j})\rangle = 0.
\end{equation}
Starting with \cref{eq:finite_gntk} and omitting $\vtheta^0$ for simplicity of notation,
\begin{align*}
    \tilde k_{\mathrm{GNN}} (G, G') & \stackrel{\text{\ref{eq:finite_gntk}}}{=}   \ggnn^T(G)\ggnn(G')\\
    & \stackrel{\text{\ref{eq:basic_def_gnn}}}{=}  \left[ \sum_{j=1}^N \frac{1}{N} \left(\gradnn^{(j)}(\bar\vh_{G,j})\right)^T \right]
    \left[ \sum_{j'=1}^N \frac{1}{\sqrt{N}} \gradnn^{(j')}(\bar\vh_{G',j'}) \right]\\
    & \stackrel{\text{\ref{eq:grad_innerprod_zero}}}{=} \frac{1}{N}  \sum_{j=1}^N \left(\gradnn^{(j)}(\bar\vh_{G,j})\right)^T 
    \gradnn^{(j)}(\bar\vh_{G',j})\\
    & = \frac{1}{N}  \sum_{j=1}^N \gradnn^T(\bar\vh_{G,j}, \vtheta^0)
    \gradnn(\bar\vh_{G',j}; \vtheta^0) \\
    & \stackrel{\text{\ref{eq:finite_ntk}}}{=} \frac{1}{N}  \sum_{j=1}^N \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j}).
\end{align*}
The next to last equation holds due to the fact that weight parameters are shared across $\nn^{(j)}$. The series of equations above prove \cref{eq:finit_gntk_ntk}. 
Plugging in the definition of the GNTK,
\begin{align*}
    \gntk(G, G') & = \lim_{m \rightarrow \infty} \frac{1}{N} \sum_{j=1}^N \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j})/m\\
    & = \frac{1}{N} \sum_{j=1}^N \lim_{m \rightarrow \infty} \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j})/m \\
    & = \frac{1}{N} \sum_{j=1}^N \ntk (\bar \vh_{G, j},\bar \vh_{G', j})
\end{align*}
where the second equality holds since $\tilde k_{\mathrm{NN}}$ is continuous, and for continues functions, limit of finite sums is equal to sum of the limits. This concludes the proof.
\end{proof}

\begin{lemma}[Sum of Reproducing Hilbert Spaces] \label{lem:sum_rkhs}
For all $1 \leq j \leq N$, suppose $\cH_j$ is a RKHS with the kernel $k_j$ defined on a domain $\cX_j$. If $\cX_i \cap \cX_j = \emptyset$ for all $i \neq j$, then the space
\[
\cH =\cH_1 + \cdots + \cH_N = \left\{\sum_{j=1}^N f_j \Big\vert\, f_j \in \cH_j\right\}
\]
together with the norm $\norm{f}^2_\cH = \sum_{j=1}^N \norm{f_j}^2_{\cH_j}$, is also a RKHS with the kernel $k: \cX \times \cX \rightarrow \sR$ where $\cX = \bigcup_{j=1}^N \cX_j$ and
\[
k(\vx, \vx') = \sum_{j = 1}^N k_j(\vx_j, \vx'_j).
\]
\end{lemma}


\begin{proof}[\textbf{Proof of \cref{lem:sum_rkhs}}]
Consider any two RKHS $\cH_{1}$ and $\cH_{2}$ with kernels $k_1$ and $k_2$, respectively. By \citet[Lemma 12.27]{wainwright2019high} the space $\cH = \cH_1 + \cH_2$, together with the norm
\[
\norm{f}^2_\cH = \min_{\substack{f_1\in \cH_1\\ f_2 \in \cH_2\\f = f_1 + f_2}} \norm{f_1}_{\cH_1} + \norm{f_2}_{\cH_2}
\]
is also a RKHS and corresponds to the kernel $k = k_1 + k_2$. Now if the two hilbert spaces are orthogonal, i.e., $\cH_1 \cap \cH_2 = \emptyset$, then any $f \in \cH$ has a unique decomposition $f = f_1+f_2$ and the norm becomes $\norm{f}^2_\cH = \norm{f_1}_{\cH_1} + \norm{f_2}_{\cH_2}$. It is straightforward to extend this result to sum of $N$ orthogonal reproducing kernel hilbert space.

By the lemma's assumptions, each two domain $\cX_i$ and $\cX_j$ are disjoint. Therefore $\cH_i \cap \cH_j = \emptyset$ for all $i \neq j$, concluding the proof.
\end{proof}

\begin{corollary}[RKHS of $\gntk$ and $\ntk$]
Mix the two lemmas above?
\end{corollary}
}

==> older drafts/Background_v1.tex <==


\section{Problem Statement}
%Let $G = (V,E)$ be an undirected graph where $V$ and $E$ denote index sets of graph nodes and edges, respectively. 
Consider $G$ to be an undirected graph and let $V(G)$ denote the set of graph nodes. Each node $u \in V(G)$ comes with a feature $\vh_u \in \cX$, where $\cX$ is a compact subset of $\R^d$.
% ===============
We use $\cN(u)$ to denote the neighborhood of node $u$ that also includes itself and define
%\begin{equation} \label{eq:node_represent}
 $   \bar \vh_u = c_u\sum_{v \in \cN(u)} \vh_v$
%\end{equation}
as the node representation obtained by aggregating and transforming the features of nodes in  $\cN(u)$.
Here, $c_u$ is a scaling factor for neighbor aggregation. As typical in Graph Convolutional Networks (GCNs) (\cite{kipf2016semi}), we consider $c_u = \norm{\sum_{v \in \cN(u)} \vh_v}_2^{-1}$, which then corresponds to averaging over neighbor features. 
% Additionally, we denote the graph feature matrix as 
% $X \in \R^{|V| \times d}$ where each row corresponds to $\vh_u$ associated with each node. The graph structure is represented via a symmetric adjacency matrix $A \in \R^{|V| \times |V|}$, and each entry $A[u,v] \in \lbrace 0,1 \rbrace$ denotes the presence (or absence) of the direct edge between node $u$ and $v$.    
% ===============
We introduce the graph bandit problem where the goal is to optimize an \emph{unknown} function $f^*: \cG \to \R$ from individual and noisy graph evaluations. 
Here, $\cG$ denotes a set of considered graphs, e.g., a finite set of graphs, and we use $N$ to denote the upper bound on the maximum number of nodes, i.e., $N \geq \max_{G \in \cG} |V_G|$. For example, in quantum chemistry, molecules are often represented as graph structures, while $f(G)$ can correspond to a molecular property of interest (e.g., atomization energy). 
The goal is to sequentially recommend molecular configurations for testing to quickly identify the most promising candidates (e.g., with the highest levels of atomization energy). Testing procedures typically require running costly experiments that result in noisy measurements.

Consequently, we consider the following learning protocol. At every time step $t \in \lbrace 1, \dots, T \rbrace$, the learner (based on the previously observed data)
selects $G_t \in \cG$, and observes a noisy function evaluation $y_t = f(G_t) + \epsilon_t$, where $\epsilon_t$ is a zero-mean $\sigma$-sub-Gaussian noise with assumed independence between time steps. Common to the bandit optimization problems, the goal of the learner is then to minimize its cumulative regret
\begin{equation}\label{eq:cumulative_regret}
    R_T = \sum_{t=1}^T \Big( f(G^*) - f(G_t) \Big),
\end{equation}
where $T$ stands for the total time horizon and $G^* \in \argmax_{G \in \cG} f(G)$. We seek algorithms that attain sub-linear regret rates in $T$, meaning that $R_T/T \to \infty$ as $T \to \infty$. However, for general graph functions, this is impossible, and hence, we make further regularity assumptions about $f$. Before we outline our main assumptions, we recall the \emph{graph neural tangent kernel} (GNTK; \cite{du2019graph}).\looseness=-1

\subsection{The Graph Neural Tangent Kernel (GNTK)}
% To learn about the unknown graph function, in this work, we use a single-block $L$-layer graph neural network (GNNs).  
In this work, we consider graph neural networks with a single graph convolutional layer and $L$ fully-connected layers that we denote as $\gnn(G; \theta): \cG \rightarrow \R$ where each fully-connected layer is of equal width $m$ and ReLU activations, defined recursively as:
\begin{equation}
    \label{eq:def_gnn}
    \begin{split}
        f^{(1)}(\bar\vh_u) &= W^{(1)}\bar\vh_u,\\
     f^{(l)}(\bar\vh_u) &= \sqrt{\frac{2}{m}} W^{(l)} \sigma_{\text{relu}}\big(f^{(l-1)}(\bar\vh_u)\big) \in \R^m,1<l\leq L\\
     \gnn(G; \theta) &=  \frac{1}{|V|}\sum_{u \in V} \sqrt{2} W^{(L+1)} \sigma_{\text{relu}}\big(f^{(L)}(\bar \vh_u)\big). 
    \end{split}
\end{equation}
Before the training, the weights $W^{(i)}$ are initialized to random matrices/vectors with standard normal i.i.d.~entries, and $\theta = (W^{(i)})_{i\leq L+1}$. 

% \begin{definition}[Graph Neural Network]
% Let $\gnn(G; \theta): \cG \rightarrow \R$ be a single-\textsc{BLOCK} GNN, followed by the simple \textsc{READOUT} operation. The \textsc{BLOCK} has $L$ fully-connected layers of equal width $m$, and ReLU activations, i.e.,
% \begin{equation*}
%     \label{eq:def_gnn}
%     \begin{split}
%         f^{(1)}(\bar\vh_u) &= W^{(1)}\bar\vh_u,\\
%      f^{(l)}(\bar\vh_u) &= \sqrt{\frac{2}{m}} W^{(l)} \sigma_{\text{relu}}\big(f^{(l-1)}(\bar\vh_u)\big) \in \R^m,\\
%      & \pushright{1<l\leq L}\\
%      \gnn(G; \theta) &=  \frac{1}{|V|}\sum_{u \in V} \sqrt{2} W^{(L+1)} \sigma_{\text{relu}}\big(f^{(L)}(\bar \vh_u)\big). 
%     \end{split}
% \end{equation*}
% The weights $W^{(i)}$ are initialized to random matrices with standard normal i.i.d.~entries, and $\theta = (W^{(i)})_{i\leq L+1}$. 
% \end{definition}


Assume that for a fixed dataset, the network is trained with gradient descent, using a small learning rate. 
Let $g_t(G) = \nabla_\theta \gnn(G; \theta^{(t)})$ denote the gradient of the network at iteration $t$. We show (in \cref{lem:GD_norm_bounds})   that as the width $m$ grows, changes in $g_t(G)$ become negligible during training. Moreover, in the infinite width limit, $\langle g_t(G), g_t(G') \rangle/m$ converges to a deterministic kernel, which is referred to as the Graph Neural Tangent Kernel (GNTK; \cite{du2019graph}). Following \citet{arora2019exact}, for any two graphs $G$ and $G'$ with $d$-dimensional node features (but potentially different number of nodes), we define the GNTK as
    \begin{equation} \label{eq:def_gntk}
    \gntk(G, G') = \lim_{m \rightarrow \infty} \frac{1}{m} \langle \nabla_\theta \gnn(G; \theta^{(0)}), \nabla_\theta \gnn(G'; \theta^{(0)}) \rangle
    \end{equation}
    where $\gnn$ is defined in \cref{eq:def_gnn}, and $\theta^{(0)}$ corresponds to the randomly initialized parameters before the training takes place.
The limiting kernel from \cref{eq:def_gntk} is deterministic and has a closed form expression. In particular, the graph neural tangent kernel of $\gnn$ can be written in terms of the neural tangent kernel $\ntk$  corresponding to $\nn$ as follows:
\begin{equation}\label{eq:gntk_vs_ntk}
        \gntk(G, G')= \frac{1}{|V||V'|} \sum_{u \in V, u'\in V'} \ntk\Big(c_u\sum_{v \in \cN(u)} \vh_v, c_u'\sum_{v' \in \cN(u')} \vh_v'\Big) =
        \frac{\sum_{u \in V, u'\in V'} \ntk(\bar\vh_u, \bar \vh_{u'})}{|V||V'|}.
\end{equation}

{\color{comment} Define $k_{NN}$ and $f_{NN}$ (maybe even in the appendix);
Shall we write that Eq. 5 follows directly from the fact that $f_{GNN}$ in our case can be written as the average of $f_{NN}$s?}

\textbf{Assumptions.} Here, we can outline the properties of $f^*$, i.e., since GNTK is defined before.

\subsection{Confidence Sets}
Motivate confidence sets: integral tool in optimization in presence of uncertainty. Online decision-making algorithms are built around uncertainty quantification via confidence sets. 

 Let $f$ be the reward function. Conditioned on the history $H_{t-1}$, for any $G \in \cG$, the set $\cC_{t-1}(G)$ defines an interval to which $f(G)$ belongs with probability greater than $1-\delta$,
 \[\sP\left(\forall G\in\cG:f(G) \in \cC_{t-1}(G)\right)\geq 1-\delta.\]
 The midpoint of this interval reflects the current knowledge of the learner, relevant for exploitation, and the width corresponds to the uncertainty, guiding further exploration.
Such sets are often constructed via calculating a midpoint $\mu_{t-1}$, and a radius $\sigma_{t-1}$. There are exceptions, i.e. likelihood ratio conf sets (e.g. Aaditya Ramdas', or Nicolas and Mojmir's work).

An approach commonly used in the kernelized bandit literature \citep{abbasiyadkori2011, srinivas2009gaussian, russo2014learning} is to pick a kernel function $k$, and  build sets of the form 
\begin{align}
    \cC_{t-1}(k;G) = [&\mu_{t-1}(k;G)-\beta_t\sigma_{t-1}(k;G), \label{eq:conf_set_def}\\ 
    &\mu_{t-1}(k;G)+\beta_t\sigma_{t-1}(k;G)]\notag
\end{align}
where the exploration coefficient $\beta_t$ depends on the desired confidence level $1-\delta$, and may be set based on the objective of the decision-making task. The functions $\mu_{t-1}$ and $\sigma_{t-1}$ are defined as
\begin{align}
    \mu_{t-1} (k;G)& = {\bm{k}}_{t-1}^T(G)({\bm K}_{t-1}+\lambda\bm{I})^{-1}\vy_{t-1}  \label{eq:GPposteriors}\\
     \sigma^2_{t-1}(k; G) & =  k(G, G) - {\bm k}^T_{t-1}(G)({\bm K}_{t-1}+\lambda\bm{I})^{-1}{\bm k}_{t-1}(G) \nonumber
\end{align}

Motivate using a GNN instead of a graph kernel: expressive power, computation advantage. Let $\bar\vg(G) = \ggnn(G; \vtheta^0)$.
We propose to instead calculate the center and width via,
\begin{equation}\label{eq:GNNposteriors}
\begin{split}
     \hat\mu_{t-1}(G) & = \gnn(G; \vtheta_{t-1}^{(J)})\\
    \hat\sigma^2_{t-1}(G) & = \frac{\bar\vg^T(G)}{\sqrt{m}}\Big(\lambda \mI + \sum_{i = 1}^{t-1} \frac{\bar \vg^T(G_i)\bar\vg(G_i)}{m}\Big)^{-1}\frac{\bar\vg(G)}{\sqrt{m}}.
\end{split}
\end{equation}





==> older drafts/Gntk_derivation.tex <==
\section{GNTK as direct sum of NTKs}
Before we dissect the connection between NTK and GNTK, we give a brief introduction into a network and its tangent kernel.

Set $\vtheta^0$ and consider the first order approximation of $\nn(\vx, \vtheta)$  and $\gnn(G, \vtheta)$ around the initial parameters $\vtheta^0$ 
\begin{align*}
    \tilde f_{\mathrm{NN}}(\vx, \vtheta) &= \gradnn^T(\vx, \vtheta^0)(\vtheta - \vtheta^0)^T,\\
    \tilde f_{\mathrm{GNN}}(G, \vtheta) &= \ggnn^T(G, \vtheta^0)(\vtheta - \vtheta^0)^T
\end{align*}
since the networks are defined to be zero at initialization. Consider any fixed dataset. Using a square loss, training with the linear model $\tilde f_{\mathrm{NN}}(\vx, \vtheta)$ (or $\tilde f_{\mathrm{GNN}}(G, \vtheta)$ resp.), is equivalent to regression with the {\em tangent kernel} \citep{jacot2018neural}, defined as 
\begin{align}
   \tilde k_{\mathrm{NN}} (\vx, \vx') & = \gradnn^T(\vx; \vtheta^0)\gradnn(\vx'; \vtheta^0),  \label{eq:finite_ntk} \\
   \tilde k_{\mathrm{GNN}} (G, G') & = \ggnn^T(G; \vtheta^0)\ggnn(G'; \vtheta^0)\label{eq:finite_gntk}
\end{align}
The tangent kernels are random, and depend on the network parameters. 
\citet{jacot2018neural} show that in the infinite width limit, $\tilde k_{\mathrm{NN}} (G, G')$ converges to a deterministic kernel, which they call the NTK,
\[
\lim_{m \rightarrow \infty} \tilde k_{\mathrm{NN}} (\vx, \vx')/m = \ntk(\vx, \vx').
\]
Similarly, we define the Graph Neural tangent kernel as 
\[
\gntk(G, G') := \lim_{m \rightarrow \infty} \tilde k_{\mathrm{GNN}} (G, G')/m.
\]
Next lemma proves that $\gntk$ is also deterministic and can be written as direct sums of $\ntk$ evaluated on aggregated features of different nodes of the graph.

\begin{lemma}\label{lem:main_gntk_ntk} Consider graphs $G$ and $G'$ with $N$ nodes. We use $\bar \vh_{G,j}$ to refer to the normalized aggregated feature of node $j$ in graph $G$.
\[
\gntk(G,G') = \frac{1}{N^2}\sum_{j = 1}^N \ntk(\bar\vh_{G,j}, \bar \vh_{G',j}) 
\]
\end{lemma}

\begin{proof}[\textbf{Proof of \cref{lem:main_gntk_ntk}}]
For any $\vtheta^0$ we first show that,
\begin{equation}\label{eq:finit_gntk_ntk}
\tilde k_{\mathrm{GNN}} (G, G') = \frac{1}{N^2} \sum_{j=1}^N \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j}).
\end{equation}
Then we take the $m \rightarrow \infty$ limit.
%We consider functions $f: \cG \rightarrow \sR$ that are invariant to how the graph nodes are indexed, i.e. invariant to permutations on the graph. In this setting, the ordering of nodes in a neighbour does not change the effect of that neighborhood on the function value either. 
The function $\gnn$ only operates on $G$ through its aggregated note features.
This motivates us to work with $\cX$ as the input domain where
\[
\cX = \left\{ \left(\bar\vh_{G,1}, \cdots,\bar\vh_{G,j}, \cdots, \bar\vh_{G,N} \right)\, \Big \vert \, \forall\, G \in \cG\right\} \subset \sR^{Nd}.
\]
Then $\cX = \bigcup_{j=1}^N \cX_j$, where $\cX_j = \{\bar \vh_{G, j} \vert \forall G \in \cG\} \subset \sR^{d, (j)}$ are $d$-dimensional subsets of $\sR^{Nd}$ and $\cX_j \cap \cX_i = \emptyset$ for all $i \neq j$.
By definition, we may write
\begin{equation}\label{eq:basic_def_gnn}
 \gnn(G; \vtheta^0) = \sum_{j=1}^N \frac{1}{N}\nn^{(j)}(\bar\vh_{G,j}; \vtheta^0)
\end{equation}
where the $(j)$ superscript is added to emphasize on the following: While the elements of $\vtheta^0$ are shared across the feed-forward networks, each $\nn^{(j)}: \cX_j \rightarrow \sR$ is zero outside $\cX_j$, if we extend its domain to $\cX$, i.e., for any $i \neq j$, 
\[
\nn^{(j)}(\bar \vh_{G, i}; \vtheta^0) = 0.
\]
Further, for any $G$, the gradient vectors $\gradnn^{(j)}(G; \vtheta^0) \in \sR^{d, (j)}$ reside in orthogonal subsets of $\sR^{Nd}$ and therefore for any $i\neq j$ and graphs $G, G' \in \cG$,
\begin{equation} \label{eq:grad_innerprod_zero}
\langle  \gradnn^{(i)}(\bar \vh_{G,i}), \gradnn^{(j)}(\bar \vh_{G',j})\rangle = 0.
\end{equation}
Starting with \cref{eq:finite_gntk} and omitting $\vtheta^0$ for simplicity of notation,
\begin{align*}
    \tilde k_{\mathrm{GNN}} (G, G') & \stackrel{\text{\ref{eq:finite_gntk}}}{=}   \ggnn^T(G)\ggnn(G')\\
    & \stackrel{\text{\ref{eq:basic_def_gnn}}}{=}  \left[ \sum_{j=1}^N \frac{1}{N} \left(\gradnn^{(j)}(\bar\vh_{G,j})\right)^T \right]
    \left[ \sum_{j'=1}^N \frac{1}{N} \gradnn^{(j')}(\bar\vh_{G',j'}) \right]\\
    & \stackrel{\text{\ref{eq:grad_innerprod_zero}}}{=} \frac{1}{N^2}  \sum_{j=1}^N \left(\gradnn^{(j)}(\bar\vh_{G,j})\right)^T 
    \gradnn^{(j)}(\bar\vh_{G',j})\\
    & = \frac{1}{N^2}  \sum_{j=1}^N \gradnn^T(\bar\vh_{G,j}, \vtheta^0)
    \gradnn(\bar\vh_{G',j}; \vtheta^0) \\
    & \stackrel{\text{\ref{eq:finite_ntk}}}{=} \frac{1}{N^2}  \sum_{j=1}^N \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j}).
\end{align*}
The next to last equation holds due to the fact that weight parameters are shared across $\nn^{(j)}$. The series of equations above prove \cref{eq:finit_gntk_ntk}. 
Plugging in the definition of the GNTK,
\begin{align*}
    \gntk(G, G') & = \lim_{m \rightarrow \infty} \frac{1}{N^2} \sum_{j=1}^N \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j})/m\\
    & = \frac{1}{N^2} \sum_{j=1}^N \lim_{m \rightarrow \infty} \tilde k_{\mathrm{NN}} (\bar \vh_{G, j},\bar \vh_{G', j})/m \\
    & = \frac{1}{N^2} \sum_{j=1}^N \ntk (\bar \vh_{G, j},\bar \vh_{G', j})
\end{align*}
where the second equality holds since $\tilde k_{\mathrm{NN}}$ is continuous, and for continues functions, limit of finite sums is equal to sum of the limits. This concludes the proof.
\end{proof}

\begin{lemma}[Sum of Reproducing Hilbert Spaces] \label{lem:sum_rkhs}
For all $1 \leq j \leq N$, suppose $\cH_j$ is a RKHS with the kernel $k_j$ defined on a domain $\cX_j$. If $\cX_i \cap \cX_j = \emptyset$ for all $i \neq j$, then the space
\[
\cH =\cH_1 + \cdots + \cH_N = \left\{\sum_{j=1}^N f_j \Big\vert\, f_j \in \cH_j\right\}
\]
together with the norm $\norm{f}^2_\cH = \sum_{j=1}^N \norm{f_j}^2_{\cH_j}$, is also a RKHS with the kernel $k: \cX \times \cX \rightarrow \sR$ where $\cX = \bigcup_{j=1}^N \cX_j$ and
\[
k(\vx, \vx') = \sum_{j = 1}^N k_j(\vx_j, \vx'_j).
\]
\end{lemma}


\begin{proof}[\textbf{Proof of \cref{lem:sum_rkhs}}]
Consider any two RKHS $\cH_{1}$ and $\cH_{2}$ with kernels $k_1$ and $k_2$, respectively. By \citet[Lemma 12.27]{wainwright2019high} the space $\cH = \cH_1 + \cH_2$, together with the norm
\[
\norm{f}^2_\cH = \min_{\substack{f_1\in \cH_1\\ f_2 \in \cH_2\\f = f_1 + f_2}} \norm{f_1}_{\cH_1} + \norm{f_2}_{\cH_2}
\]
is also a RKHS and corresponds to the kernel $k = k_1 + k_2$. Now if the two hilbert spaces are orthogonal, i.e., $\cH_1 \cap \cH_2 = \emptyset$, then any $f \in \cH$ has a unique decomposition $f = f_1+f_2$ and the norm becomes $\norm{f}^2_\cH = \norm{f_1}_{\cH_1} + \norm{f_2}_{\cH_2}$. It is straightforward to extend this result to sum of $N$ orthogonal reproducing kernel hilbert space.

By the lemma's assumptions, each two domain $\cX_i$ and $\cX_j$ are disjoint. Therefore $\cH_i \cap \cH_j = \emptyset$ for all $i \neq j$, concluding the proof.
\end{proof}

\begin{corollary}[RKHS of $\gntk$ and $\ntk$]
Mix the two lemmas above?
\end{corollary}

==> older drafts/Perm_invar.tex <==
% \subsection{A Theoretical Comment on Permutation Invariance}

% Neural decision-making algorithms use a neural network as an approximator for a reward functions which lies in some hypothesis space. This hypothesis space is often assumed to be an RKHS.

% We compare two scenarios. We first consider a neural network that ignores the graph structure and takes the stacked vector of node features as the input. Then we show that by using a GNN and thereby leveraging the graph structure, the working hypothesis space {\em shrinks} in dimensionality by a factor of $N!$. 

% \paragraph{Ignoring Structure}
% Define $\vz_G \in \sS^{Nd-1}$ as the normalized concatenated vector of all node features,
% \[
% \vz_G = \left( \frac{1}{c_G} \vh_{u}\right)_{u \in V(G)}.
% \]
% where $c^2_G = \sum_{u \in V(G)} \norm{\vh_u}_2^2$.
% We consider using $\nn(\vz_G; \vtheta): \sS^{Nd-1}\rightarrow \sR$ to estimate the reward function.
% We discuss how this choice affects of the hypothesis space of the learner when solving the bandit task. In the infinite-width limit, $\nn$ lies in $\cH_\ntk$, where
% \begin{equation*}
%     \ntk(\vz_G, \vz_{G'}) = \sum_{k=0}^\infty \mu_k \sum_{j=1}^{N(Nd,k)} Y_{j,k}(\vz_G)Y_{j,k}(\vz_{G'}).
% \end{equation*}
% The spherical harmonic polynomials $\{\bar Y_{j,k}\}_{j=1}^{N(Nd, k)}$ span $\cH_\ntk$.
% We conclude that the hypothesis space of a learner which uses $\nn(\vz_G)$ as an approximator of the reward, is the span of spherical harmonics on $\sS^{Nd-1}$.

% \paragraph{Leveraging Sturcture} Define $\vx_G \in \sS^{Nd-1}$ as the stacked vector of all aggregated node features,
% \[
% \vx_G = \left(\frac{1}{N}\bar\vh_{u}\right)_{u \in V(G)}.
% \]
% Note that by definition of $\bar\vh_u$, for any graph $G \in \cG$
% \[
% \norm{\vx_G}_2^2 = \frac{1}{N}\sum_{u \in V(G)} \norm{\bar \vh_u}_2^2 = 1.
% \]
% Using this notation, we re-write the definition of $\gnn$. For simplicity, the next equation is written for the $2$-layer network. It should be clear from \cref{eq:def_gnn} how also applies to an $L$-layer GNN.
% \[
% \gnn(\vx_G) = \gnn(G; \vtheta) =  \frac{1}{N}\sum_{j = 1}^N \frac{2}{\sqrt{m}} \sum_{i=1}^{m} \alpha_i \sigma(\langle \vw_i, N\vx_{G, j:j+d}\rangle)
% \]
% For any width $m$, we can show that $\gnn: \sS^{Nd-1}\rightarrow R$, lies in $L^2(\sS^{Nd-1})$, with the uniform measure used for integration. 

% {\color{comment}[TODO. This would be done via \cref{eq:gnn_vs_nn} and using the fact that the NN lies in this space.]}

% The graph neural network has a particular structure and so lies within a smaller permutation-invariant subset of $L^2(\sS^{Nd-1})$. Let $P_{N}$ denote the group of permutations over a set of size $N$.
% We then define the group of block-permutations operating on $\sS^{Nd-1}$ as
% \[
% P_{N,\mathrm{block}} = \left\{ p: p(\vx_G) = \left(\frac{1}{N}\bar\vh_{q(u)}\right)_{u \in V(G)} , q \in P_{N}\right\}
% \]
% It immediately follows that $\gnn$ is block-permutation invariant, or in other words, invariant to permutations of the node indices.
% \[
% \gnn(\vx_G) = \frac{1}{N!} \sum_{p \in P_{N,\mathrm{block}} } \gnn(p \cdot \vx_G)
% \]
% We can then show that {\color{comment}[TODO. Easy.]}
% \[
% \gntk(\vx_{G}, \vx_{G'}) =  \frac{1}{N!} \sum_{p \in P_{N,\mathrm{block}} } \gntk(p \cdot \vx_G, \vx_{G'}).
% \]
% Group-invariant functions in $L^2(\sS^{Nd-1})$, such as $\gnn$, have a simpler characterization. \citet{bietti2021sample} show that the set of $P$-invariant functions is spanned by the $P$-invariant spherical harmonics. This invariance reduces the dimensionality of such harmonics by a factor of $\vert P \vert$.

% The graph neural networks of our interest are $P_{N,\mathrm{block}}$-invariant, and correspond to a kernel function which may be written as,
% \begin{equation*}
%     \gntk(\vx_{G}, \vx_{G'})  = \sum_{k=0}^\infty \bar \mu_k \sum_{j=1}^{\bar N(Nd,k)} \bar Y_{j,k}(\vx)\bar Y_{j,k}(\vx')
% \end{equation*}
% where $\{\bar Y_{j,k}\}_{j=1}^{N(Nd, k)}$ are the  $P_{N,\mathrm{block}}$-invariant spherical harmonics of degree $k$ and
% \[
% \frac{\bar N(Nd,k)}{N(Nd,k)} \leq \frac{1}{N!}.
% \]
% {\color{comment}
% I'm not making any comment about $\bar\mu_k$ and how they decay. I'm trying to see what can be said. It seems to me that \citet{bietti2021sample} doesn't give a direct solution. It gives an integral (right after eqation 4) which we might be able to calculate using the technique in \citet{bietti2020deep}. If we can show that $\bar \mu_k$ decays like the NTK's $\mu_k$, then we will this $N!$ shrinking in our other bounds as well.

% This all being said, I still need to think more and understand what's happening better. This analysis feels handwavy. Talking about the eigenfunctions without discussing the decay of eigenvalues does not seem ok.}
% \paragraph{Conclusion}




% Let $V_{d,k}$ be the space of degree-$k$ polynomials that are orthogonal to the space of polynomials of degree less than $k$, defined on $\sS^{d-1}$. Then $V_{d,k}(\cC_d)$ denotes the subspace of $V_{d,k}$ that is also $\cC_d$-invariant. 

% The NTK kernel satisfies the Mercer condition and has the following Mercer decomposition \citep{bietti2020deep},
% \begin{equation*}
%     k_{\text{NTK}}(\vx, \vx') = \sum_{k=0}^\infty \mu_k \sum_{j=1}^{N(d,k)} Y_{j,k}(\vx)Y_{j,k}(\vx')
% \end{equation*}
% where $\{Y_{j,k}\}_{j \leq N(d,k)}$ form an orthonormal basis for $V_{d,k}$. \citet{bietti2020deep} further show that $Y_{j,k}$ is the $j$-th spherical harmonic polynomial of degree $k$, and $N(d,k) = \text{dim}(V_{d,k})$ gives  the total count of such polynomials, where
% \[N(d, k) = \frac{2k+d-2}{k} \binom{k+d-3}{d-2}.\]
% For any integer $k$, it also holds that \citep{bietti2020deep}
% \begin{equation}\label{eq:gegenbauer}
% \sum_{j=1}^{N(d,k)} Y_{j,k}(\vx)Y_{j,k}(\vx') = N(d,k) Q^{(d)}_k(\vx^T\vx')
% \end{equation}
% where $Q_k^{(d)}$ is the $k$-th Gegenbauer polynomial in dimension $d$. It follows from Equation \ref{eq:gntk_vs_ntk} that $k_{\text{CNTK}}$ is also Mercer. 

% Assume that it has a Mercer decomposition of the form
% \[
% k_{\text{CNTK}}(\vx, \vx') =  \sum_{k=0}^\infty \bar \mu_k \sum_{j=1}^{\bar N(d,k)} \bar Y_{j,k}(\vx)\bar Y_{j,k}(\vx').
% \]
%  We now proceed to identify $\bar Y_{j,k}$ and calculate $\bar N(d,k)$.

==> older drafts/Sec3_Theory.tex <==
\section{Theory}


\subsection{Information Gain}

\begin{lemma}[Information Gain bound]
\[
\gamma_{T, \mathrm{gntk}} \leq c \gamma_{T,\mathrm{ntk}}
\]
\end{lemma}

\subsection{Confidence Bound}
We give a confidence interval for norm-bounded functions residing in $\cH_{\gntk}$, around $ \gnn(G; \vtheta^{(J)}_t ) $ a GNN trained for $J$ steps using the history $H_t$.

 \begin{lemma}[Confidence interval for $\gnn$ around $f^*$]\label{lem:CI_gnn_truereward}
Set $\delta \in (0,1)$.
Suppose $f^* \in \cH_{\gntk}$ and has a bounded norm $\norm{f^*}_{\gntk}\leq B$. Samples of $f$ are observed with zero-mean sub-Gaussian noise of variance proxy $\sigma^2$. 
 Let $H_t = \{(G_i, y_i)\}_{i \leq t}$ denote the history and assume that $(G_i)_{i \leq t}$ and $(\varepsilon_i)_{i\leq t}$ are statistically independent. 
Set $J>1$ and choose the width such that
\begin{align*}
         m =   \poly \left(t, L, \vert \cG\vert,\lambda, \lambda_0^{-1}, \log( N/\delta)\right),
         \end{align*}
         %\poly\left(t, L, |\cG|, \lambda,B^{-1}, \lambda_0^{-1}, \log(N/\delta)\right)
and $\eta = C(LmtN^2+m\lambda)^{-1}$ with some universal constant $C$. Then for a graph $G \in \cG$, with probability of at least $1-\delta$, 
\begin{equation*}
    \begin{split}
        \vert \gnn(G; \vtheta^{(J)}_t )- f^*(G) \vert \leq \hat\sigma_{t}(G) \Bigg[ \sqrt{2}B + &\frac{\lambda}{\sigma}\sqrt{2\log2/\delta} +  \sqrt{\frac{2tB}{m\eta\lambda}}\big( \sqrt{2} + (1-m\eta\lambda )^{J/2}\big) \Bigg] \\
        & + \tilde C L^3\left(\frac{tB}{m \lambda}\right)^{2/3} \sqrt{m \log m}
    \end{split}
\end{equation*}

for some constant $\bar C$, where is $\hat\sigma_{t}$ defined as in \cref{alg:gnnalg}.

\end{lemma}
Proof for Lemma \ref{lem:CI_gnn_truereward} is given in \cref{app:main_CI_proof}.

\begin{theorem}[Regret Bound for \gnnalg]\label{thm:simple_regret} Set $\delta \in (0,1)$.
Suppose $f^* \in \cH_{\gntk}$ and has a bounded norm $\norm{f^*}_{\gntk}\leq B$. Samples of $f$ are observed with zero-mean sub-Gaussian noise of variance proxy $\sigma^2$. Set $J>1$ and choose the width such that
\begin{align*}
         m =   \poly \left(t, L, \vert \cG\vert, \lambda, B, \lambda_0^{-1}, \log( N/\delta)\right),
         \end{align*}
         %\poly\left(t, L, |\cG|, \lambda,B^{-1}, \lambda_0^{-1}, \log(N/\delta)\right)
and $\eta = C(Lmt+m\lambda)^{-1}$ with some universal constant $C$. Then with probability greater than $1-\delta$, the simple regret of \gnnalg satisfies
\begin{align*}
    r_T \leq \cO \left( \sqrt{\frac{\gamma_T}{T}} \left( B + \frac{\lambda}{\sigma}\sqrt{\vert \cG\vert \log 1/\delta}\right)\right)
\end{align*}
\end{theorem}
The proof is given in \cref{app:simple_regret}.



==> older drafts/story2.tex <==
{\color{old}
\section{Permutation invariant additive model}
}
% We start with a setup that assumes no geometrical symmetries over the graph domain. We characterize the graph by the $Nd$-dimensional feature vector $\vh_{G} = (\vh_{G,j})_{j=1}^N$ together with its adjacency matrix.

% \paragraph{Domain}

% We assume that $\bar \vh_{G, j} \in \cX^{(j)}$ where $\cX^{(j)}$ is finite. Similarly, we let $\bar \vh_G = (\bar \vh_{G,j})_{j=1}^N \in \sR^{Nd}$.
% Then,
% $$\cG = \{G: \,  \vert V(G)\vert =  N \text{ and } \forall j \in V(G):  \bar \vh_{G,j} \in \cX^{(j)}\}.$$ 

% {\color{comment}
% \textbf{Possible interpretation}: The key take away is that when defining the domain, we don't assume that features corresponding to each node are not necessary corresponding to the same property. If in the definition of the graph we assumed that for all $1\leq j\leq N$, $\vh_{G,j} \in \sR^d$, we would be assuming that the same set of features are given for all nodes. But we don't do this. {\em We impose all the desirable symmetries by making assumptions about the reward function.}
% }

\begin{theorem}\label{thm:MIG_bargntk}
Suppose the observation noise is i.i.d., and drawn from a zero-mean sub-gaussian with variance proxy $\lambda>0$, and the input domain is $\cG$. Then the maximum information gain associated with $\gntk$  is bounded by
\[
        \gamma_T = \mathcal{O}\left(  N \left( \frac{c(d, L)T}{N! \log (1+ T/\lambda)} \right)^{\frac{d-1}{d}}
         \log\left( 1
          + \frac{NT}{\sigma^{2}}\left( \frac{c(d, L)T}{N!\log (1+ T/\lambda)} \right)^{\frac{d-1}{d}} \right)\right)
\]
\end{theorem}
To prove theorem \cref{thm:MIG_bargntk} we first characterize $\bar k$ in terms of its eigenvalues and eigenfunctions.
\begin{lemma} \label{lem:gntkbar_mercer}
 The permutation invariant additive kernel $\bar k$ can be decomposed as
 \begin{equation*}
    \bar k(G, G') =  \sum_{r=0}^\infty \frac{\lambda_r}{N} \sum_{s=1}^{\bar N(d,r)} \sum_{j=1}^N \bar Y^{(j)}_{ s,r}(\bar \vh_{G})\bar Y^{(j)}_{ s,r}(\bar \vh_{G'})
\end{equation*}
where $\lambda_{\mathrm{GNN}, k}$ are the eigenvalues of $\ntk$. The algebraic multiplicity is $\bar N(d,k) \leq \tfrac{N}{N!} N(d,k)$, and the eigenfunctions $\{\bar Y^{(j)}_{s,r}\}_{s \leq \bar N(d,r), j \leq N}$ form an orthonormal basis for the space of $P_{N,d}$-invariant degree-$r$ polynomials on $\sS^{Nd-1}$. 
\end{lemma}

\begin{proof}[\textbf{Proof of \cref{thm:MIG_bargntk}}]
The permutation invariant additive kernel is Mercer by Lemma \ref{lem:gntkbar_mercer}. Which implies that we may repeat the steps taken in the proof of Theorem \ref{thm:MIG_gntk_basic}. To avoid confusion, we use the \emph{``bar''} notation to indicate the permutation-invariant counterpart of the parameters from that proof. The GNTK and $\bar k$ share the same eigenvalues. The eigenfunctions of $\bar k$ also bounded by one over the hyper sphere. The changes to the analysis will make up for the difference between algebraic multiplicities $N(d,r)$ and $\bar N(d,r)$, which comes into effect only for calculating $\text{tr}(\bar K_{O,X_T})$. 
For $\bar k$ we would have,
\begin{align*}
    \text{tr}\left(\bar K_{O,X_T}\right) & \leq T  \sum_{r\geq D+1}\lambda_r \bar N(d,r) \\
    & \leq  T  \sum_{r\geq D+1}\lambda_r N(d, r)/N!  \\
    & \leq \frac{T c(d, L)}{N!} \sum_{r\geq D+1} r^{-2} \\
    & \leq \frac{c(d, L)}{N!D} 
\end{align*} 
Equivalent to Equation \ref{eq:infogain_last} we may write,
\[
    I(\vy_T; \vf_T)  \leq \frac{1}{2} \tilde D \log\left(  1 +  \frac{T\lambda^{-1}}{\tilde D}\right) + \frac{T}{2} \log\left( 1 + \frac{c(d, L)}{N!D} \right).
\]
where similar to the proof of Theorem \ref{thm:MIG_gntk_basic}, we have defined $\tilde D = \Theta(\bar D^{d-1})$. For the first term to be larger than the second, $\tilde D$ has to be set to
\[
\tilde D =\Big\lceil N \left(\frac{c(d, L) T}{N!\log (1+ T/\lambda)}\right)^{\frac{d-1}{d}}\Big\rceil
\]
which then concludes the proof. 
\end{proof}
